Decoupled classifiers for fair and efficient machine learning

When it is ethical and legal to use a sensitive attribute (such as gender or race) in machine learning systems, the question remains how to do so. We show that the naive application of machine learning algorithms using sensitive features leads to an inherent tradeoff in accuracy between groups. We provide a simple and efficient decoupling technique, that can be added on top of any black-box machine learning algorithm, to learn different classifiers for different groups. Transfer learning is used to mitigate the problem of having too little data on any one group. The method can apply to a range of fairness criteria. In particular, we require the application designer to specify as joint loss function that makes explicit the trade-off between fairness and accuracy. Our reduction is shown to efficiently find the minimum loss as long as the objective has a certain natural monotonicity property which may be of independent interest in the study of fairness in algorithms.

==> scraps.tex <==
\section{Model}
We begin by analyzing the case where the loss is simply average error (or more generally average loss), which is the starting point and predominant approach within ML systems. What we show is that fairness issues arise as accuracy tradeoffs between groups even when one is using an average error model, and we show how decoupling helps avoid these tradeoffs. In Section \ref{sec:Loss}, we analyze a general notion of loss that accounts for differences between groups. 

Let $\mathcal{X} = \mathcal{X}_1 \cup \mathcal{X}_2 \cup \ldots \cup \mathcal{X}_K$ be the set of possible {\em examples} partitioned into $K$ disjoint groups, and let $g:\mathcal{X}\rightarrow \{1,2,\ldots,K\}$ denote the function that determines which group in which example $x$ belongs so $x\in \mathcal{X}_{g(x)}$. There are sets of labels $\mathcal{Y}\subseteq \reals$ and predictions $\hat{\mathcal{Y}}\subseteq\reals$. There is a joint distribution $\mathcal{D}$ over $\mathcal{X}\times \mathcal{Y}$.% and a sequence of $n$ training examples $(x_1, y_1),\ldots, (x_n,y_n)\in \mathcal{X} \times \mathcal{Y}$. 

We have a family $\mathcal{C}$ of {\em classifiers} $c:\mathcal{X} \rightarrow \hat{\mathcal{Y}}$, where classifications are in a set $\hat{\mathcal{Y}}$.  For instance, if $\mathcal{X} \subseteq \reals^d$, the set of linear classifiers is, $$\mathcal{C}_{\text{lin}} = \{ c(x)=w\cdot x+b ~|~b \in \reals, w\in \reals^d\}.$$ When  $\mathcal{Y}$ is continuous, these are often called regressors, but we will use the term classifier for consistency throughout.

The goal is to minimize average error rate, or more generally minimize {\em expected loss} $\E[\ell(y, c(x))]$ over $(x,y)\sim \mathcal{D}$, for a given loss function $\ell:\mathcal{Y} \times \hat{\mathcal{Y}} \rightarrow \reals$, such as {\em squared error} $\ell(y,\hat{y}) = (y-\hat{y})^2$ or {\em absolute error} $\ell(y,\hat{y}) = |y-\hat{y}|$. For $\mathcal{Y}, \hat{\mathcal{Y}} \subseteq [-1,1]$ it is also common to consider {\em log loss}, $\ell(y,\hat{y}) = -\log_2 \frac{1+y\hat{y}}{2}$. 

For each group, a potentially different classifier may have better loss. Hence, by being forced to use a single classifier, one may suboptimal on each group. 
We quantify this tradeoff by the following quantity\footnote{Formally, to ensure that max and min are well-defined, one may restrict $\mathcal{C}, \mathcal{X}, \mathcal{Y}$ to be finite sets (such as $b$-bit numbers or vectors), or one can replace max/min with sup/inf and impose standard measure-theoretic assumptions.}:
\begin{equation}\label{cost}
\text{cost-of-coupling}(\mathcal{C}, \ell) = \max_{\mathcal{D}} \left( \min_{c \in \mathcal{C}}{\E}_{(x,y)\sim \mathcal{D}}[\ell(y, c(x))]-
\min_{\vec{c} \in \mathcal{C}^K}{\E}_{(x,y)\sim \mathcal{D}}[\ell(y, c_{g(x)}(x))] \right)
\end{equation}
Note that these quantities are defined with respect to expected loss, i.e., as if we had infinite data -- finite sample algorithms will be considered in Section \red{?}. It is easy to see that the cost of coupling is non-negative. This is because one could simply choose the same estimator $\vec{c}=(c,c,\ldots,c)$ for each group in the decoupled classifier. 

%CD: I don't want us to say that being wrong can be viewed as being unfair. We don't need to do this, and work by, eg., the philosopher Deborah Hellman sharply calls this into question.
%The cost of coupling can be viewed as a measure of classifier unfairness in the case where misclassifications are viewed as unfair. For instance, if a positive classification is favorable (such as admission to an organization) and a positive label $y$ indicates that the person would have been successful had they been given the positive classification, then any false negative is arguably unfair to the person who was not admitted. A classifier that fails to minimize errors...

%Which the accuracy of one or more groups is compromised to accommodate accurate classification of another group. 


A solution is to consider {\em decoupled} classifiers $\gamma_{\vec{c}}$ for $\vec{c} \in \mathcal{C}^K$, where $f_k$ is the estimator for group $k$, and $\gamma_{\vec{c}}(x)=f_{g(x)}(x)$.  For family $\mathcal{C}$, we define the set of decoupled classifiers is denoted $\gamma(\mathcal{C})=\{\gamma_{\vec{c}}~|~\vec{c} \in \mathcal{C}^K\}.$ A family $\mathcal{C}$ is called {\em decoupled} if $\gamma(\mathcal{C})=\mathcal{C}$. 

Theorem \ref{thm:tradeoff} shows that the cost of coupling is zero if and only if the family is decoupled. Moreover, common families of classifiers are not naturally decoupled and can exhibit tradeoffs in accuracy across groups that are large in magnitude. In Section \ref{sec:tradeoff}, we define the families of classifiers described in the theorem and give its proof. 

Thusfar, fairness is modeled by accuracy within each group. For instance, if a minority group can be better classified by their own classifier than having to use the same classifier as the majority group, one may say that it is unfair to them to be forced to be evaluated by the same classifier as the majority group. We later illustrate such a situation in Figure \red{?}. We now consider more general models of loss that account combine accuracy with notions of fairness.

% First, we show that decoupling removes some unnecessary tradeoffs in loss across groups. %Why should the accuracy on one group suffer to compensate for accuracy on another group?
% However, is there any point in decoupling estimators? Perhaps the estimator naturally accounts for differences in groups, i.e., $\mathcal{C}=\bigl\{\gamma_{\vec{c}}~|~\vec{c}\in \mathcal{C}^K\bigr\}$. In fact, we show that this is not the case for most of the estimators in use today, including linear models (e.g., linear regression), generalized linear (e.g., logistic regression), and support vector machines (e.g., SVR with a Gaussian kernel). Furthermore, for the more recently popular regression trees and forests (e.g., random forests), and neural networks, we show that as long as they are of sub-exponential size, the decoupled versions are strictly richer than the coupled versions.

% Third, we give a simple, general black-box reduction to fitting decoupled estimators given a fitting procedure. The reduction aims to compensate for the natural tendency for decoupled classifiers to overfit more than their coupled counterparts, due to decreased data. In experiments on a number of datasets from \url{openml.org}, we find that on some problems, accuracy tradeoffs can be mitigated by decoupling.

% Up to this point, we consider a model in which one is solely concerned with accuracy, group-by-group, and decoupling helps remove accuracy tradeoffs across groups. Such tradeoffs are one type of unfairness. But an estimator with greater accuracy, even if it is more accurate on each and every group, may lead to arguably decreased ``fairness'' under certain metrics. 

\subsection{Fairness and accuracy loss}




\subsection{Weak monotonicity}


\section{Blah}\label{sec:Loss}

We next consider models of fairness, distinguishing fairness {\em outcome metrics} from {\em classifier objectives}. Metrics measure the fairness of the outcomes, whereas classifier objectives are designed so fairness is increased when they are improved. We note that naively misusing outcome metrics as classifier objectives can lead to undesirable classifiers. Consider the following two quantities:
The first one is often useful as a metric, any differences in false negative rates may reflect an underlying unfairness in the classifier or in society on the whole. Minimizing it may lead to unfairly increasing the false negative rates in one group simply to 




one unfairness metric might be,  which captures the difference in false negative rates. This difference may reflect a bias favoring accuracy in the majority class, but it may also reflect an underlying unfairness that exists before the tests. In other words, as a metric, it may be perfect

This difference may point to something unfair about the classifier, or it may reflect the unfairness prevalence

However, using such a metric

Now, an example of a monotonic objective would be:
$$,$$
which 


if one insists on using the same test across sexes, then one must 


in the example of admission, if we have more perfectly accurate measurements of one group and no data on another group, this may reflect an {\em inherent} societal unfairness that should not be blamed on an ML classifier and which cannot be corrected by a classifier (other than by random admission). Such a metric measure differences in false negative rates. 




If the estimation procedure naturally partitions the data by group, then the best 


